SoK: Decoding the Enigma of Encrypted Network Traffic Classifiers

The adoption of modern encryption protocols such as TLS 1.3 has significantly challenged traditional network traffic classification (NTC) methods. As a consequence, researchers are increasingly turning to machine learning (ML) approaches to overcome these obstacles. In this paper, we comprehensively analyze ML-based NTC studies, developing a taxonomy of their design choices, benchmarking suites, and prevalent assumptions impacting classifier performance. Through this systematization, we demonstrate widespread reliance on outdated datasets, oversights in design choices, and the consequences of unsubstantiated assumptions. Our evaluation reveals that the majority of proposed encrypted traffic classifiers have mistakenly utilized unencrypted traffic due to the use of legacy datasets. Furthermore, by conducting 348 feature occlusion experiments on state-of-the-art classifiers, we show how oversights in NTC design choices lead to overfitting, and validate or refute prevailing assumptions with empirical evidence. By highlighting lessons learned, we offer strategic insights, identify emerging research directions, and recommend best practices to support the development of real-world applicable NTC methodologies.

==> tables/3_overfitting_sample_scenario.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{2.7}

    \caption{Overfitting sample scenario}
    \label{tab:3_overfitting_sample_scenario}
    
    \centering
    \small

    \resizebox{\columnwidth}{!}{
        \rowcolors{2}{}{lightgray}        
        
        \begin{tabular}{*{1}{L{3.2cm}}*{2}{L{2.55cm}}l} % Left align the columns
            
            \toprule
            
                \multicolumn{1}{c}{\textbf{Feature}} & 
                \multicolumn{1}{l}{\textbf{Training Samples}} & 
                \multicolumn{1}{l}{\textbf{Testing Samples}} & 
                \multicolumn{1}{l}{\textbf{Unseen}} \\ 
            
            \midrule
            
                IP ID  & 
                 \makecell[l]{P15 = 0x\textbf{b0}a0  \\[3pt] P39 = 0x\textbf{b0}ac} & 
                 \makecell[l]{P29 = 0x\textbf{b0}a7  \\[3pt] P45 = 0x\textbf{b0}af} & 
                 0xd5e6 \\[3pt] 
                
                IP Header Checksum & 
                \makecell[l]{P15 = 0x\textbf{f4}44  \\[3pt] P39 = 0x\textbf{f4}5a} & 
                \makecell[l]{P29 = 0x\textbf{f4}5f  \\[3pt] P45 = 0x\textbf{f4}55} & 
                0xc39e \\[3pt] 
                
                TCP Seq. No. & 
                \makecell[l]{P15 = 0x\textbf{418d4}7a1  \\[3pt] P39 = 0x\textbf{418d4}cab} & 
                \makecell[l]{P29 = 0x\textbf{418d4}754  \\[3pt] P45 = 0x\textbf{418d4}cc3} & 
                0x3c49ff50 \\[3pt]
                
                TCP Ack. No. & 
                \makecell[l]{P15 = 0x\textbf{03c2}8800  \\[3pt] P39 = 0x\textbf{03c2}a0e7} & 
                \makecell[l]{P29 = 0x\textbf{03c2}a09f  \\[3pt] P45 = 0x\textbf{03c2}a101} & 
                0x0d238466 \\[3pt]
                
                TCP Window Size & 
                \makecell[l]{P15 = 0x\textbf{02}03  \\[3pt] P39 = 0x\textbf{02}e5} & 
                \makecell[l]{P29 = 0x\textbf{02}e5  \\[3pt] P45 = 0x\textbf{02}e5} & 
                0x00ec \\[3pt]
                
                TCP Options = TSval & 
                \makecell[l]{P15 = 0x\textbf{04ad}86d0  \\[3pt] P39 = 0x\textbf{04ad}8934} &
                \makecell[l]{P29 = 0x\textbf{04ad}86eb  \\[3pt] P45 = 0x\textbf{04ad}90f5} & 
                0x3afaf1de \\[3pt]
                
                TCP Options = TSerc & 
                \makecell[l]{P15 = 0x\textbf{3c4}3ba79  \\[3pt] P39 = 0x\textbf{3c4}3d15f} & 
                \makecell[l]{P29 = 0x\textbf{3c4}3ba8a  \\[3pt] P45 = 0x\textbf{3c4}4190c} & 
                0x2d53588d \\[3pt] 
            
            \bottomrule

            \addlinespace[-3pt]
            \multicolumn{4}{l}{ 

                \begin{tabular}[l]{@{}l@{}}

                    \rowcolor{white}
                    
                    \large\textbf{P$n$}=Packet number $n$ \\
                    
                \end{tabular}
                
            }
        
        \end{tabular}
    }
\end{table}

==> tables/5_datasets_and_classes.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\footnotesize

    \caption{Datasets and classes used in evaluation}
    \label{tab:5_datasets_and_classes}
    
    \centering

    \resizebox{\columnwidth}{!}{
        \rowcolors{2}{}{lightgray}        
        
        \begin{tabular}{c*{2}{L{3cm}}}
        
            \toprule
                
                \multicolumn{1}{c}{\textbf{\#}} & 
                \multicolumn{1}{c}{\textbf{CipherSpectrum}} & 
                \multicolumn{1}{c}{\textbf{CSTNET-TLS1.3}} \\ 

            \midrule

                1 &
                cloudfront.net &
                apple.com \\

                2 &
                doubleclick.net &
                cisco.com \\

                3 &
                gmx.net &
                cloudflare.com \\

                4 &
                google.com &
                facebook.com \\

                5 &
                google-analytics.com &
                github.com \\

                6 &
                hotjar.com &
                icloud.com \\

                7 &
                hubspot.com &
                netflix.com \\

                8 &
                robinhood.com &
                nike.com \\

                9 &
                segment.com &
                nvidia.com \\
                
                10 &
                sharethis.com &
                yahoo.com \\

                
            
            \bottomrule
        
        \end{tabular}
    }
\end{table}
